Edge Generation Scheduling for DAG Tasks Using Deep Reinforcement Learning

Directed acyclic graph (DAG) tasks are currently adopted in the real-time domain to model complex applications from the automotive, avionics, and industrial domains that implement their functionalities through chains of intercommunicating tasks. This paper studies the problem of scheduling real-time DAG tasks by presenting a novel schedulability test based on the concept of trivial schedulability. Using this schedulability test, we propose a new DAG scheduling framework (edge generation scheduling -- EGS) that attempts to minimize the DAG width by iteratively generating edges while guaranteeing the deadline constraint. We study how to efficiently solve the problem of generating edges by developing a deep reinforcement learning algorithm combined with a graph representation neural network to learn an efficient edge generation policy for EGS. We evaluate the effectiveness of the proposed algorithm by comparing it with state-of-the-art DAG scheduling heuristics and an optimal mixed-integer linear programming baseline. Experimental results show that the proposed algorithm outperforms the state-of-the-art by requiring fewer processors to schedule the same DAG tasks. The code is available at https://github.com/binqi-sun/egs.

==> algorithms/ppo.tex <==
{
% \SetAlCapFnt{\small}
% \SetAlCapNameFnt{\small}
% \SetAlFnt{\small}
\begin{algorithm} [htb]
    \caption{The PPO training process}
    \label{alg:ppo}
    \For{$i\gets 1$ \KwTo $iters$}{
        $Rollout \gets \varnothing$\; 
        $s_t \gets$ Sample a DAG task from train set\;
        \For(\tcp*[f]{collect phase}){$t\gets 1$ \KwTo $L$}{
            % Sample a DAG task from the train set\;
            % Observe the current state $s_t$\;
            % $s_t \gets (\mathcal{G},D)$\;
            $a_t \gets$ Sample from policy $\pi_{\theta_i}(s_t)$\;
            % Select an action $a_t$ by sampling from policy $\pi_{\theta_i}$\;
            $Rollout \gets Rollout \cup \{(s_t, a_t, R(s_t,a_t), r_t(\theta_i))\}$\;
            
            % Add $(s_t, a_t, R(s_t,a_t), r_t(\theta_i))$ to the rollout\;
            % Collect $T$ experiences by interacting the actor network with the environment for $T$ steps\;
            % Compute advantage estimates based on the collected experiences and the critic network\;
            $s_t \gets$ Transit to next state with action $a_t$\;
            \If{terminate}{
                $s_t \gets$ Sample a DAG task from train set\;
            }
        }
        \For(\tcp*[f]{train phase}){$k\gets 1$ \KwTo $K$}{
            \For{$\mathcal{B} \in Rollout$}{
                Update $\pi_\theta$ and $V^\pi_\phi$ with \eqref{eq:loss_c} and \eqref{eq:loss_a}\;
            }
        }
        % with $K$ epochs and minibatch size $|\mathbb{B}| \leq NT$;\
    }
\end{algorithm}
}

==> figures/encoder.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{figures/encoder.pdf}
\caption{Illustration of the encoder layer.}
\label{fig:encoder}
\end{figure}

==> figures/nn_overall.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=\linewidth]{figures/nn_overall_fig.pdf}
\caption{Illustration of the actor and critic network.}
\label{fig:nn_overall}
\end{figure}

==> figures/res_opt.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.85\linewidth]{figures/opt_gap.pdf}
\caption{Optimality gap when $n \leq 20$.}
\label{fig:res_opt}
\end{figure}

==> tables/training_time.tex <==
\begin{table} [ht]
\center
\begin{threeparttable}
\caption{PPO hyper-parameters.}\label{tab:train_time}

\setlength{\tabcolsep}{\mytabcolsepsmall}
\begin{tabular}{l|ll}
\hline
Experiment & Convergence time & training iterations \\
\hline

$\max n = 20$ &  hours & $100$
$\max n = 50$ &  hours & $200$
$\max n = 100$ &  hours & $350$
$\max n = 150$ &  & $300$

\hline

\end{tabular}

\end{threeparttable}

\end{table}
